Feasible Automata for Two-Variable Logic with Successor on Data Words

We introduce an automata model for data words, that is words that carry at each position a symbol from a finite alphabet and a value from an unbounded data domain. The model is (semantically) a restriction of data automata, introduced by Bojanczyk, et. al. in 2006, therefore it is called weak data automata. It is strictly less expressive than data automata and the expressive power is incomparable with register automata. The expressive power of weak data automata corresponds exactly to existential monadic second order logic with successor +1 and data value equality \sim, EMSO2(+1,\sim). It follows from previous work, David, et. al. in 2010, that the nonemptiness problem for weak data automata can be decided in 2-NEXPTIME. Furthermore, we study weak B\"uchi automata on data omega-strings. They can be characterized by the extension of EMSO2(+1,\sim) with existential quantifiers for infinite sets. Finally, the same complexity bound for its nonemptiness problem is established by a nondeterministic polynomial time reduction to the nonemptiness problem of weak data automata.

==> LATA-commands.tex <==
\newcounter{CommentCounter}
\newcommand{\mcomment}[2]{%
  \stepcounter{CommentCounter}%
  {\bf$^{(\arabic{CommentCounter})}$}%
  \marginpar{$^{({\bf{\arabic{CommentCounter}}})}${\small #1: #2}}}

%%%%%%%%%%%%%%%%%%%%%%
%%                   comments                            %%
%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\acomment}[2]{\ \\ \fbox{\parbox{\linewidth}{{\sc #1}:\\ #2}}}
\newcommand{\ahmet}[1]{\acomment{Ahmet}{#1}}
\newcommand{\thomas}[1]{\acomment{Thomas}{#1}}
\newcommand{\tony}[1]{\acomment{Tony}{#1}}

\newcommand{\mahmet}[1]{\mcomment{Ahmet}{#1}}
\newcommand{\mthomas}[1]{\mcomment{Thomas}{#1}}
\newcommand{\mtony}[1]{\mcomment{Tony}{#1}}
\newcommand{\leaveout}[1]{}

%%%%%%%%%%%%%%%%%%%%%%
%%            theorem environments              %%
%%%%%%%%%%%%%%%%%%%%%%
% \newtheorem{claim}{Claim}
% \newtheorem{definition}{Definition}
% \newtheorem{theorem}{Theorem}
% \newtheorem{proposition}{Proposition}
% \newtheorem{remark}{Remark}
%\newtheorem{eg}{Example}

% \newcommand{\proof}{{\scshape\noindent Proof.\quad}}
% \newcommand{\qed}{\hfill\rule{1ex}{1em}\penalty-1000{\par\medskip}}

% \newenvironment{example}{\eg \em}{\vspace{0.5 em}}

%%%%%%%%%Commands%%%%%%%%%%%%%%%

\newcommand{\dataU}{\mbox{$U^{\sim}$}}
\newcommand {\dataX}{\mbox{$X^{\sim}$}}
\newcommand{\dataS}{\mbox{$S^{\sim}$}}
\newcommand {\dataY}{\mbox{$Y^{\sim}$}}
\newcommand{\labeling}[2]{\mbox{$l_{#1}(#2)$}}
\newcommand{\stringproj}[2]{\mbox{$s(#1,#2)$}}
\newcommand{\classpos}[2]{\mbox{$p_{\textrm{\scriptsize class}}(#1,#2)$}}
\newcommand{\wordpos}[3]{\mbox{$p_{\textrm{\scriptsize word}}(#1,#2,#3)$}}
\newcommand {\classpltl}{\mbox{\textrm{DataClassPLTL}}}
\newcommand {\pointsto}[1]{\mbox{\textit{pointsto-#1}}}
\newcommand {\bitat}[2]{\mbox{\textit{bit-#1-#2}}}
%%%%%%%%%Commands%%%%%%%%%%%%



\newcommand{\completeLTL}
{\mbox{$\textrm{LTL}[\Diamond^{w},\Diamond^{s},\ttX_{\sim},\ttX_{\nsim}]$}}
\newcommand{\completeLTLstrong}
{\mbox{$\textrm{LTL}[\Diamond^{s},\ttX_{\sim},\ttX_{\nsim}]$}}
\newcommand{\diamondLTL}{\mbox{$\textrm{LTL}[\Diamond]$}}
\newcommand{\weakdiamondLTL}{\mbox{$\textrm{LTL}[\Diamond^{w}]$}}
\newcommand{\strongdiamondLTL}{\mbox{$\textrm{LTL}[\Diamond^{s}]$}}

%%%%%%%%%%%%%%%%% SYMBOLS %%%%%

\newcommand{\fD}{\mbox{$\mathfrak{D}$}}

\newcommand{\nn}{\mbox{${\mathbb N}$}}

\newcommand{\ttX}{\mbox{$\texttt{X}$}}
\newcommand{\ttY}{\mbox{$\texttt{Y}$}}
\newcommand{\ttU}{\mbox{$\texttt{U}$}}
\newcommand{\ttS}{\mbox{$\texttt{S}$}}
\newcommand{\ttR}{\mbox{$\texttt{R}$}}
\newcommand{\ttF}{\mbox{$\texttt{F}$}}
\newcommand{\ttG}{\mbox{$\texttt{G}$}}
\newcommand{\suc}{\mbox{$\texttt{Suc}$}}

\newcommand{\profile}[1]{\mbox{Profile$(#1)$}}

\newcommand{\LL}{{\cal L}}

\newcommand{\bbS}{\mbox{$\mathbb{S}$}}
\newcommand{\sbbS}{\mbox{\scriptsize $\mathbb{S}$}}

\renewcommand{\AA}{\mbox{$\mathcal{A}$}\xspace}
\newcommand{\BB}{\mbox{$\mathcal{B}$}}
\newcommand{\CC}{\mbox{$\mathcal{C}$}\xspace}
\newcommand{\FF}{\mbox{$\mathcal{F}$}}
\renewcommand{\LL}{\mbox{$\mathcal{L}$}}
\newcommand{\MM}{\mbox{$\mathcal{M}$}}
\newcommand{\OO}{\mbox{$\mathcal{S}$}}
\newcommand{\QQ}{\mbox{$\mathcal{Q}$}}
\newcommand{\RR}{\mbox{$\mathcal{R}$}}
\renewcommand{\SS}{\mbox{$\mathcal{S}$}}
\newcommand{\TT}{\mbox{$\mathcal{T}$}}
\newcommand{\ZZ}{\mbox{$\mathcal{Z}$}}


\newcommand{\sCC}{\mbox{\scriptsize $\mathcal{C}$}}
\newcommand{\sFF}{\mbox{\scriptsize $\mathcal{F}$}}
\newcommand{\sRR}{\mbox{\scriptsize $\mathcal{R}$}}
\newcommand{\sSS}{\mbox{\scriptsize $\mathcal{S}$}}

\newcommand{\True}{\mbox{$\textsf{True}$}}
\newcommand{\False}{\mbox{$\textsf{False}$}}

\newcommand{\ckey}{\mbox{$\textsf{key}$}}


\newcommand{\closure}{\mbox{$\textsf{Cl}$}}
\newcommand{\sclosure}{\mbox{\tiny $\textsf{Cl}$}}

\newcommand{\atoms}{\mbox{$\textsf{Atoms}$}}
\newcommand{\PTIME}{\mbox{$\textsf{PTIME}$}}
\newcommand{\NP}{\mbox{$\textsf{NP}$}}
\newcommand{\NEXPTIME}{\mbox{$\textsf{NEXPTIME}$}\xspace}
\newcommand{\EXPTIME}{\mbox{$\textsf{EXPTIME}$}}
\newcommand{\EXPSPACE}{\mbox{$\textsf{EXPSPACE}$}}
\newcommand{\PSPACE}{\mbox{$\textsf{PSPACE}$}}

\newcommand{\sffin}{\mbox{$\textsf{fin}$}}
\newcommand{\sfinf}{\mbox{$\textsf{inf}$}}


\newcommand{\sfProj}{\mbox{$\textsf{Str}$}}
\newcommand{\proj}{\sfProj}
\newcommand{\sfInf}{\mbox{$\textsf{Inf}$}}
\newcommand{\sfProfile}{{\sf Profile}}
%\newcommand{\profile}{\sfProfile}
\newcommand{\sfParikh}{\mbox{$\textsf{Parikh}$}}
\newcommand{\sfImage}{\mbox{$\textsf{Image}$}}
\newcommand{\sfprofile}{\mbox{$\textsf{profile}$}}

\newcommand{\key}{\mbox{$\textsf{Key}$}}

\newcommand{\tsfImage}{\mbox{\tiny $\textsf{Image}$}}

\newcommand{\sfZonal}{\mbox{\sf Zonal}}
\newcommand{\tsfZonal}{\mbox{\sf {\tiny Zonal}}}
\newcommand{\tscZonal}{\mbox{$\textsc{\tiny zonal}$}}

\newcommand{\tsffin}{\mbox{\tiny $\textsf{fin}$}}
\newcommand{\tsfinf}{\mbox{\tiny $\textsf{inf}$}}

\newcommand{\FO}{\mbox{$\textsf{FO}$}}
\newcommand{\MSO}{\mbox{$\textsf{MSO}$}}
%\newcommand{\EMSO}{\mbox{$\exists\textsf{MSO}$}}
\newcommand{\EMSO}{\mbox{$\textsf{EMSO}$}}
\newcommand{\EIMSO}{\mbox{$\textsf{E$_\infty$MSO}$}}

\newcommand{\LTL}{\mbox{$\textsf{LTL}$}}

\newcommand{\rhoOmega}{\rho^{\omega}}

%%%%%% Added by Thomas

\newcommand{\nc}{\newcommand}
\nc{\bigO}{\ensuremath{{\cal O}}}
\newcommand{\Lab}{\ensuremath{L_{a*b}}\xspace}
\newcommand{\Labo}{\ensuremath{L_{a<b}}\xspace}

%corrections
\setul{}{0.3mm}
\setstcolor{red}
\newcommand{\oldnew}[3]{{\textcolor{blue}{\setlength{\fboxsep}{1pt}\fbox{\small #1}}} \st{#2} \textcolor{blue}{#3}}
\newcommand{\moldnew}[3]{\textcolor{red}{\acomment{#1 DELETED:}{#2}} \textcolor{blue}{#3}}
% For submission change into
%\renewcommand{\oldnew}[3]{#3}
% Changes by Ahmet[old text]{new text}
\nc{\aon}[2][]{\oldnew{A}{#1}{#2}} 
% Changes by Tony[old text]{new text}
\nc{\ton}[2][]{\oldnew{TT}{#1}{#2}}
% Changes by Thomas[old text]{new text}
\nc{\thon}[2][]{\oldnew{TS}{#1}{#2}}

%\nc{\shortorlong}[2]{#1}  % For submission
\nc{\shortorlong}[2]{#2}  % For long version - however compare with appendix

\nc{\qhat}{\ensuremath{\hat{q}}\xspace}
\newcommand{\aproj}{\mbox{$\textsf{a-Proj}$}}
\nc{\mblack}{\mbox{black}}
\nc{\myellow}{\mbox{yellow}}
\nc{\mblue}{\mbox{blue}}
\nc{\mwhite}{\mbox{white}}

%opening=

==> LATA-conclusion.tex <==
\section{Conclusion}
\label{s:conclusion}


We conclude this paper with two open problems for future directions.
An obvious open problem is the exact complexity of the nonemptiness
problem for weak data automata. 
The current 2-\NEXPTIME yields a 3-\NEXPTIME upper bound for the
satisfiability problem for $\EMSO^2(+1,\sim)$. However, as it is known
that this problem can be solved in 2-\NEXPTIME~\cite{NiewerthS11}, some
room for improvement is left.

Another interesting question is how our results can be applied to
temporal logics. In~\cite{demri-lazic-tocl}, a restriction of \ \LTL \
with one register, {\em simple} \ \LTL, was considered with the same expressive power as
some two variable logic. We conjecture that there is a correspondence
between our logics and the restriction of simple \ \LTL \ to
the operators $X$, $X^{-1}$ and an operator that allows navigation to
some other position.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

